CipherDAug: Ciphertext based Data Augmentation for Neural Machine Translation

We propose a novel data-augmentation technique for neural machine translation based on ROT-$k$ ciphertexts. ROT-$k$ is a simple letter substitution cipher that replaces a letter in the plaintext with the $k$th letter after it in the alphabet. We first generate multiple ROT-$k$ ciphertexts using different values of $k$ for the plaintext which is the source side of the parallel data. We then leverage this enciphered training data along with the original parallel data via multi-source training to improve neural machine translation. Our method, CipherDAug, uses a co-regularization-inspired training procedure, requires no external data sources other than the original training data, and uses a standard Transformer to outperform strong data augmentation techniques on several datasets by a significant margin. This technique combines easily with existing approaches to data augmentation, and yields particularly strong results in low-resource settings.

==> orig_intro.tex <==
Neural machine translation (NMT) \cite{bahdanau2015attn, vaswani2017attention} systems today are capable of learning powerful representational spaces \cite{raganato2018analysis, voita2019analyzing, kudugunta2019investigating} and easily scale to a large number of langauges and massive data \cite{aharoni-etal-2019-massively}. However, due to the model capacity required to capture such complex representations, NMT is often susceptible to memorization and poor generalization. Data augmentation is a simple,  regularization-inspired technique to improve the generalization of NMT models.

%Typically, data augmentation algorithms generate extra data points from the empirically observed training set to train subsequent a translation model.

\begin{figure}
    \centering
    \includegraphics[scale=0.65]{figures/cipher-intro.pdf}
    \caption{ROT-k encipherment}
    \label{fig:rotk}
\end{figure}

Back-translation \cite{sennrich2016improving} is arguably the most widely used data augmentation strategy for NMT. Although the original approach utilizes external monolingual data to augment parallel training data \cite{edunov2018understanding, xia2019generalized}, in-domain back-translation of the original parallel data has also shown promise \cite{nguyen19datadiverse}. While such methods yield lexically diverse training data, it is often semantically poor owing to the technique's dependence on trained models that are not impervious to errors themselves \cite{edunov2018understanding}.
The second most common approach is based on input perturbations (replacement/deletion/insertion) as either a continuous \cite{gao-etal-2019-soft, liu-etal-2021-counterfactual, takase-kiyono-2021-rethinking} or a discreet \cite{belinkov2018synthetic} function of words \cite{sennrich-etal-2016-edinburgh} or spans \cite{guo-etal-2020-sequence, wu-etal-2021-mixseq}. Even though most methods based on word replacement improve the generalization of NMT models, they either ignore the contexts of replaced words (Switchout, RAML) or fracture the alignment between source and target sequences, both detrimental for generating high-quality data.

Data augmentation in NMT is challenging because it is nontrivial to find simple data equivalencies. The augmented data must balance between lexical diversity, syntactic similarity, and semantic correlation to existing data. Even a slight modification to a sequence can result in drastic and impermissible changes to its syntax and semantics, and any alteration to a source sentence might require corresponding changes to its translation.

% Weaver 1949:
% this process [decipherment] ma[kes] use of frequencies of letters, letter combinations, [...] etc., which are to some significant degree independent of the language used. 
In this paper, we focus on augmenting existing training sets without adding any external data, monolingual or otherwise. We propose a novel data-augmentation technique for neural machine translation which employs simple ROT-$k$ ciphers. A ROT-$k$ cipher (Figure~\ref{fig:rotk}) is a substitution cipher that replaces a letter in the input (the so-called \textit{plaintext}) with the $k$th letter after it in the alphabet. Our technique creates multiple ROT-$k$ enciphered copies of the source side of a parallel dataset, each copy using a different value of $k$. This results in lexically diverse (almost non-overlapping) source sentences, and unlike existing data-augmentation techniques,  guarantees complete syntactic and semantic equivalence to the original source language.
